Globular Cluster UVIT Legacy Survey (GlobULeS) $-$ II. Evolutionary status of hot stars in M3 and M13

We present a far-ultraviolet (FUV) study of hot stellar populations in the second parameter pair globular clusters (GCs) M3 and M13, as a part of the Globular cluster UVIT Legacy Survey program (GlobULeS). We use observations made with F148W and F169M filters of the Ultraviolet Imaging Telescope (UVIT) onboard {\em AstroSat} along with ground-based data (UBVRI filters), {\em Hubble Space Telescope (HST)} GC catalogue, and {\em Gaia} EDR3 catalogue. Based on the FUV-optical colour-magnitude diagrams, we classify the sources into the horizontal branch (HB) stars, post-HB stars, and hot white dwarfs (WDs) in both the GCs. The comparison of synthetic and observed colours of the observed HB stars suggests that the mass-loss at the red giant branch (RGB) and He spread in both clusters have a simultaneous effect on the different HB distributions detected in M3 and M13, such that, HB stars of M13 require a larger spread in He (${\rm 0.247-0.310}$) than those of M3 (${\rm Y= 0.252-0.266}$). The evolutionary status of HB stars, post-HB stars, and WDs are studied using SED fit parameters and theoretical evolutionary tracks on the H-R diagram. We found that the observed post-HB stars have evolved from zero-age HB (ZAHB) stars of the mass range $0.48-0.55$ \Msun\ in M3 and M13. We detect 24 WD candidates in each cluster having ${\rm \log(L_{bol}/L_\odot)}$ in the range $-0.8$ to $+0.6$ and ${\rm \log(T_{eff}/K)}$ in the range of 4.2 to 5.0. Placing the WDs on the H-R diagram and comparing them with models suggest that M13 has a population of low-mass WDs, probably originating from binary evolution.

==> journals.tex <==
 %Inherited from mn-jour.bib
\def\aao{{AAO Newsl.}~}
\def\aavso{{AAVSO Newsl.}~}
\def\acta{{Acta Astron.}~}
\def\aaguv{{Acta Astron. Geophys. Univ. Comenianae}~}
\def\actastsin{{Acta Astron. Sin.}~}
\def\actapsin{{Acta Astrophys. Sin.}~}
\def\agg{{Acta Geod. Geophys.}~}
\def\ags{{Acta Geophys. Sin.}~}
\def\appsb{{Acta Phys. Pol., Ser. B}~}
\def\atash{{Acta Tech. Acad. Sci. Hung.}~}
\def\advp{{Adv. Phys.}~}
\def\advsr{{Adv. Space Res.}~}
\def\aip{{AIP Conf. Proc.}~}
\def\aavsob{{Am. Assoc. Variable Star Obs. Bull.}~}
\def\aavsoc{{Am. Assoc. Variable Star Obs. Circ.}~}
\def\amjp{{Am. J. Phys.}~}
\def\aatar{{Anglo--Aust. Telesc., Annu. Rep.}~}
\def\ag{{Ann. Geophys.}~}
\def\araa{{ARA\&A}~} % "Ann. Rev. Astron. Astrophys."
\def\apl{{Ann. Phys. (Leipzig)}~}
\def\apny{{Ann. Phys. (N.Y.)}~}
\def\app{{Ann. Phys. (Paris)}~}
\def\ao{{Appl. Opt.}~}
\def\appl{{Appl. Phys. Lett.}~}
\def\apb{{Appl. Phys., B}~}
\def\as{{Appl. Spectrosc.}~}
\def\ahes{{Arch. Hist. Exact Sci.}~}
\def\archuk{{Archeoastronomy (U.K.)}~}
\def\asbts{{Archenhold--Sternw. Berlin--Treptow, Sonderdr.}~}
\def\asbtvs{{Archenhold--Sternw. Berlin--Treptow, Vortr. Schr.}~}
\def\aonaicnl{{Arecibo Obs./NAIC, Newsl.}~}
\def\artsat{{Artif. Satell.}~}
\def\aiisao{{Astrofiz. Issled. Izv. Spets. Astrofiz. Obs.}~}
\def\af{{Afz}~} % "Astrofizika"
\def\aa{{A\&A}~} % "Astron. Astrophys."
\def\aap{{A\&A}~} % "Astron. Astrophys."
\def\aapr{{A\&AR}~} % "Astron. Astrophys. Rev."
\def\aas{{A\&AS}~} % "Astron. Astrophys. Suppl. Ser."
\def\abco{{Astron. Bull. (Carter Obs.)}~}
\def\agas{{Astron. Ges., Abstr. Ser.}~}
\def\asther{{Astron. Her.}~}
\def\aiubc{{Astron. Inst. Univ. Brno, Contrib.}~}
\def\astj{{AJ}~} % "Astron. J."
\def\aj{{AJ}~} % "Astron. J."
\def\an{{Astron. Nachr.}~}
\def\astnow{{Astron. Now}~}
\def\astraum{{Astron. Raumfahrt}~}
\def\astriha{{Astron. Rechen-Inst.Heidelb., Mitt., Ser. A}~}
\def\astrihb{{Astron. Rechen-Inst.Heidelb., Mitt., Ser. B}~}
\def\astschu{{Astron. Sch.}~}
\def\asttid{{Astron. Tidsskr.}~}
\def\asttsir{{Astron. Tsirk.}~}
\def\astvest{{Astron. Vestn.}~}
\def\astzh{{AZh}~} % "Astron. Zh."
\def\astuai{{Astronomia UAI}~}
\def\astie{{Astronomie}~}
\def\asty{{Astronomy}~}
\def\apj{{ApJ}~} % "Astrophys. J."
\def\apjl{{ApJL}~} % "Astrophys. J. Lett."
\def\apjss{{ApJS}~} % "Astrophys. J. Suppl. Ser."
\def\apjs{{ApJS}~} % "Astrophys. J. Suppl. Ser."
\def\aplc{{Astrophys. Lett. Commun.}~}
\def\apss{{Astrophys. Space. Sci.}~}
\def\apss{{Astrophys. Space. Sci.}~}
\def\ap{{Astrophysics}~}
\def\aanlsor{{Atti Accad. Naz. Lincei, Ser. Ottava, Rend.}~}
\def\ajast{{Aust. J. Astron.}~}
\def\ajp{{Aust. J. Phys.}~}
\def\bavm{{BAV Mitt.}~}
\def\bavr{{BAV Rundbrief}~}
\def\bbsag{{BBSAG Bull.}~}
\def\bestarnl{{Be Star Newsl.}~}
\def\bildw{{Bild Wiss.}~}
\def\bipm{{BIPM Circ. T}~}
\def\boaumkt{{Biul. Obs. Astron. Uniw. M. Kopernika Toruniu}~}
\def\boe{{Bol. Obs. Ebro}~}
\def\broa{{Bol. ROA}~}
%\def\blm{{Boundary-Layer Meteorol.}~}
%\def\boop{{Boyden Obs., Occas. Publ.}~}
%\def\bastac{{Br. Astron. Assoc. Circ.}~}
%\def\bjp{{Bulg. J. Phys.}~}
%\def\baas{{BAAS}~} % "Bull. Am. Astron. Soc."
%\def\baps{{Bull. Am. Phys. Soc.}~}
%\def\bafoev{{Bull. Assoc. Fr. Obs. Etoiles Variables}~}
%\def\bastic{{Bull. Astron. Inst. Czech.}~}
%\def\basi{{Bull. Astron. Soc. India}~}
%\def\bain{{Bull. Astron. Inst. Netherlands}~}
%\def\bcao{{Bull. Crimean Astrophys. Obs.}~}
%\def\bgsi{{Bull. Geogr. Surv. Inst.}~}
%\def\bicds{{Bull. Inf. Cent. Donn\'ees Stellaires}~}
%\def\boab{{Bull. Obs. Astron. Belgr.}~}
%\def\crassgvs{{C. R. Acad. Sci., S\'er. G\'en., Vie Sci.}~}
%\def\crassii{{C. R. Acad. Sci., II}~}
%\def\cjp{{Can. J. Phys.}~}
%\def\cm{{Celest. Mech.}~}
%\def\cassos{{Cent. Astron. Sci. Spat., Obs. Sol.}~}
%\def\cent{{Centaurus}~}
%\def\cpl{{Chem. Phys. Lett.}~}
%\def\chinaa{{Chin. Astron. Astrophys.}~}
%\def\chinp{{Chin. Phys.}~}
%\def\chinpl{{Chin. Phys. Lett.}~}
%\def\ciel{{Ciel}~}
%\def\cielt{{Ciel Terre}~}
%\def\ccotl{{Circ. Czech. Obs. Time Lattiude}~}
%\def\cinf{{Circ. Inf.}~}
%\def\ctls{{Circ. Time Latitude Serv.}~}
%\def\cqg{{Classical Quantum Gravity}~}
%\def\cast{{Comments Astrophys.}~}
%\def\cnpp{{Comments Nucl. Part. Phys.}~}
%\def\cppcf{{Comments Plasma Phys. Controlled Fusion}~}
%\def\cfsua{{Commun. Fac. Sci. Univ. Ankara, Ser. A2, A3}~}
%\def\cko{{Commun. Konkoly Obs.}~}
%\def\cmp{{Commun. Math. Phys.}~}
%\def\culo{{Commun. Univ. Lond. Obs.}~}
%\def\comp{{Comput. Phys.}~}
%\def\compcom{{Comput. Phys. Commun.}~}
%\def\cp{{Contemp. Phys.}~}
%\def\caosp{{Contrib. Astron. Obs. Skalnat\'e Pleso}~}
%\def\cap{{Contrib. Atmos. Phys.}~}
%\def\cdaut{{Contrib. Dep. Astron., Univ. Tokyo}~}
%\def\clo{{Contrib. Lick Obs.}~}
%\def\cncopb{{Contrib. Nicholas Copernicus Obs. Planetarium Brno}~}
%\def\cnjro{{Contrib. Nizamiah Japal-Rangapur Obs.}~}
%\def\cpp{{Contrib. Plasma Phys.}~}
%\def\cvvo{{Contrib. Van Vleck Obs.}~}
%\def\cr{{Cosmic Res.}~}
%\def\cryo{{Cryogenics}~}
%\def\czjp{{Czech. J. Phys., Sect. B}~}
%\def\drho{{Data Rep. Hydrogr. Obs., Ser. Astron. Geod.}~}
%\def\dgkbawb{{Dtsch. Geod. Komm. Bayer. Akad. Wiss., Reihe B}~}
%\def\dgkbawc{{Dtsch. Geod. Komm. Bayer. Akad. Wiss., Reihe C}~}
%\def\dgkbawe{{Dtsch. Geod. Komm. Bayer. Akad. Wiss., Reihe E}~}
%\def\epsl{{Earth Planet. Sci. Lett.}~}
%\def\erb{{Earth Rotation Bull.}~}
%\def\emp{{Earth, Moon, Planets}~}
%\def\esrev{{Earth--Sci. Rev.}~}
%\def\esab{{ESA Bull.}~}
%\def\esaiuenl{{ESA IUE Newsl.}~}
%\def\esaj{{ESA J.}~}
%\def\esoar{{ESO Ann. Rep.}~}
%\def\ejp{{Eur. J. Phys.}~}
%\def\epl{{Europhys. Lett.}~}
%\def\epn{{Europhys. News}~}
%\def\expast{{Exp. Astron.}~}
%\def\fiz{{Fizika}~}
%\def\fortp{{Fortschr. Phys.}~}
%\def\fp{{Found. Phys.}~}
%\def\funcp{{Fundam. Cosmic Phys.}~}
%\def\gaab{{G.~A.A.B.}~}
%\def\gast{{G. Astron.}~}
%\def\gem{{Gemini}~}
%\def\grg{{Gen. Relativ. Gravitation}~}
%\def\gca{{Geochim. Cosmochim. Acta}~}
%\def\ga{{Geomagn. Aehron.}~}
%\def\gafd{{Geophys. Astrophys. Fluid Dyn.}~}
%\def\gj{{Geophys. J.}~}
%\def\grl{{Geophys. Res. Lett.}~}
%\def\geo{{Geophysics}~}
%\def\geos{{GEOS Circ.}~}
%\def\gbg{{Gerlands Beitr. Geophys.}~}
%\def\heav{{Heavens}~}
%\def\hpa{{Helv. Phys. Acta}~}
%\def\hepnp{{High Energ. Phys. Nucl. Phys.}~}
%\def\hob{{Hvar Obs. Bull.}~}
%\def\hi{{Hyperfine Interact.}~}
%\def\iappp{{I.A.P.P.P. Commun.}~}
%\def\iauc{{IAU Circ.}~}
%\def\iauib{{IAU Inf. Bull.}~}
%\def\icarus{{Icarus}~}
%\def\i3etm{{IEEE Trans. Magn.}~}
%\def\i3etns{{IEEE Trans. Nucl. Sci.}~}
%\def\i3etps{{IEEE Trans. Plasma Sci.}~}
%\def\iersbb{{IERS Bull. B}~}
%\def\iersba{{IERS Bull.--A}~}
%\def\ijpap{{Indian J. Pure Appl. Phys.}~}
%\def\ijrsp{{Indian J. Radio Space Phys.}~}
%\def\ibvs{{Inf. Bull. Variable Stars}~}
%\def\iaatub{{Inst. Astron. Astrophys. Tech. Univ. Berlin, Mitt.}~}
%\def\iag{{Inst. Astron. Geod., Univ. Madr., Publ.}~}
%\def\ia{{Inst. Astron., Univ. Camb., Annu. Rep.}~}
%\def\icq{{Int. Comet Q.}~}
%\def\ijimw{{Int. J. Infrared Millimeter Waves}~}
%\def\ijmp{{Int. J. Mod. Phys. A}~}
%\def\ijtp{{Int. J. Theor. Phys.}~}
%\def\ip{{Inverse Probl.}~}
%\def\iastj{{Ir. Astron. J.}~}
%\def\iris{{IRIS Bull. A}~}
%\def\iskz{{Issled. Solntsa Krasnykh Zvezd}~}
%\def\intsa{{Itogi Nauki Tekh., Ser. Astron.}~}
%\def\intsppk{{Itogi NAuki Tekh., Ser. Plazmennye Protsessy Kosmose}~}
%\def\iaoe{{Izv. Astron. Obs. Ehngel'gardt.}~}
%\def\ikao{{Izv. Krym. Astrofiz. Obs.}~}
%\def\ivuzr{{Izv. Vyssch. Uchebn. Zaved., Radiofiz.}~}
%\def\jasa{{J. Acoust. Soc. Am.}~}
%\def\jaavso{{J. Am. Assoc. Variable Star Obs.}~}
%\def\jam{{J. Appl. Meteorol.}~}
%\def\jap{{J. Appl. Phys.}~}
%\def\jastf{{J. Astron. Fr.}~}
%\def\japast{{JA\&A}~} % "J. Astrophys. Astron."
%\def\jas{{J. Atmos. Sci.}~}
%\def\jatp{{J. Atmos. Terr. Phys.}~}
%\def\jbasta{{J. Br. Astron. Assoc.}~}
%\def\jbis{{J. Br. Interplanet. Soc.}~}
%\def\jcp{{J. Chem. Phys.}~}
\def\jcap{{JCAP}~} % "Jounal of Cosmology and Astroparticle Physics"
%\def\jcomp{{J. Comp. Phys.}~}
%\def\jel{{J. Electrostat.}~}
%\def\jfseu{{J. Fac Sci., Ege Univ., Ser. A}~}
%\def\jfm{{J. Fluid Mech.}~}
%\def\jgr{{J. Geophys. Res.}~}
%\def\jhast{{J. Hist. Astron.}~}
%\def\jms{{J. Mater. Sci.}~}
%\def\jmp{{J. Math. Phys.}~}
%\def\jmo{{J. Mod. Opt.}~}
%\def\jop{{J. Opt. (Paris)}~}
%\def\josaa{{J. Opt. Soc. Am. A}~}
%\def\josab{{J. Opt. Soc. Am. B}~}
%\def\jp{{J. Phys.}~}
%\def\jpa{{J. Phys. A}~}
%\def\jpb{{J. Phys. B}~}
%\def\jpd{{J. Phys. D}~}
%\def\jpe{{J. Phys. E}~}
%\def\jpg{{J. Phys. G}~}
%\def\jpsj{{J. Phys. Soc. Jpn.}~}
%\def\jpp{{J. Plasma Phys.}~}
%\def\jqsrt{{J. Quant. Spectrosc. Radiat. Transfer}~}
%\def\jrasc{{J. R. Astron. Soc. Can.}~}
%\def\jsp{{J. Stat. Phys.}~}
%\def\jvst{{J. Vac. Sci. Technol., A}~}
%\def\jetpl{{JETP Lett.}~}
%\def\jhatd{{Johns Hopkins APL Tech. Dig.}~}
%\def\jjap1{{Jpn. J. Appl. Phys., Part 1}~}
%\def\jjap2{{Jpn. J. Appl. Phys., Part 2}~}
%\def\kai{{Kapteyn Astron. Inst., Annu. Rep.}~}
%\def\kexto{{Kexue Tongbao}~}
%\def\kfnt{{Kinematika Fiz. Nebesn. Tel}~}
%\def\kob{{Kodaikanal Obs. Bull.}~}
%\def\kt{{Komet. Tsirk.}~}
%\def\ki{{Kosm. Issled.}~}
%\def\koz{{Kozmos}~}
%\def\kpm{{KPM}~}
%\def\lo{{Laser Optoelektron.}~}
%\def\latc{{Latitude Circ.}~}
%\def\lest{{LEST Found., Annu. Rep.}~}
%\def\lmp{{Lett. Math. Phys.}~}
%\def\lob{{Lick Obs. Bull.}~}
%\def\mg{{Manuscr. Geod.}~}
%\def\ml{{Mater. Lett.}~}
%\def\mrb{{Mater. Res. Bull.}~}
%\def\mfs{{Mem. Fac. Sci., Kyoto Univ., Ser. Phys., Astrophys., Geophys., Chem.}~}
%\def\memras{{Mem. R. Astron. Soc.}~}
\def\msai{{Mem. Soc. Astron. Ital.}~}
%\def\merc{{Mercury}~}
%\def\mess{{Messenger}~}
%\def\met{{Meteoritics}~}
%\def\metka{{Meteoritika}~}
%\def\metro{{Metrologica}~}
%\def\mpb{{Minor Planet Bull.}~}
%\def\mpc{{Minor Planet Circ.}~}
%\def\masbt{{Mitt. Archenold--Sternw. Berlin Treptow}~}
%\def\mag{{Mitt. Astron. Ges.}~}
%\def\mlotud{{Mitt. Lohrmann--Obs., Tech. Univ. Dresden}~}
%\def\mss{{Mitt. Sternw. Sonneberg}~}
%\def\mvs{{Mitt. Ver{\"a}nderliche Sterne}~}
%\def\mzpe{{Mitt. Zentralinst. Phys. Erde}~}
%\def\mpla{{Mod. Phys. Lett. A}~}
\def\mn{{MNRAS}~} % "Mon. Not. R. Astron. Soc."
\def\mnras{{MNRAS}~} % "Mon. Not. R. Astron. Soc."
%\def\mnassa{{Mon. Notes Astron. Soc. S. Afr.}~}
%\def\nint{{Nablyud. Iskusstv. Nebesn. Tel.}~}
%\def\nogb{{Nachr. Olbers--Ges. Bremen}~}
%\def\naoj{{Natl. Astron. Obs. (Jpn.), Repr.}~}
%\def\ng{{Natl. Geogr.}~}
%\def\nraoa{{Natl. Radio Astron. Obs., Repr., Ser. A}~}
%\def\nraob{{Natl. Radio Astron. Obs., Repr., Ser. B}~}
\def\nat{{Nature}~} % "Nature"
%\def\natwis{{Naturwissenschaften}~}
%\def\ni{{Nauchn. Inf.}~}
%\def\nlasny{{News Lett. Astron. Soc. N.Y.}~}
%\def\nrodaour{{Nizamiah Rangapur Obs. Dep. Astron., Osmania Univ., Repr.}~}
%\def\nraow{{NRAO Workshop}~}
%\def\nimpra{{Nucl. Instrum. Methods Phys. Res., Sect. A}~}
%\def\nimprb{{Nucl. Instrum. Methods Phys. Res., Sect. B}~}
%\def\npa{{Nucl. Phys. A}~}
%\def\npb{{Nucl. Phys. B, Part. Phys.}~}
%\def\nca{{Nuovo Cimento A}~}
%\def\ncb{{Nuovo Cimento B}~}
%\def\ncc{{Nuovo Cimento C}~}
%\def\ot{{Obs. Trav.}~}
%\def\obs{{Observatory}~}
%\def\onl{{Occultation Newsl.}~}
%\def\ozvp{{{\"O}sterr. Z. Vermessungswes. Photogramm.}~}
%\def\oc{{Opt. Commun.}~}
%\def\oe{{Opt. Eng.}~}
%\def\olt{{Opt. Laser Technol.}~}
%\def\ol{{Opt. Lett.}~}
%\def\on{{Opt. News}~}
%\def\os{{Opt. Spectrosc.}~}
%\def\optik{{Optik}~}
%\def\ofeb{{Origins Life Evol. Biosphere}~}
%\def\orion{{Orion}~}
%\def\orione{{Orione}~}
%\def\oac{{Oss. Astrofis. Catania, Pubbl.}~}
%\def\pz{{Perem. Zvezdy}~}
%\def\pb{{Phys. Bl.}~}
%\def\pcm{{Phys. Chem. Miner.}~}
%\def\pfa{{Phys. Fluids, A}~}
%\def\pfb{{Phys. Fluids, B}~}
%\def\pla{{Phys. Lett. A}~}
%\def\plb{{Phys. Lett. B}~}
%\def\pr{{Phys. Rep.}~}
\def\physrep{{Phys. Rep.}~}
\def\pra{{Phys. Rev. A}~}
\def\prb{{Phys. Rev. B}~}
\def\prc{{Phys. Rev. C}~}
\def\prd{{Phys. Rev. D}~}
\def\prl{{Phys. Rev. Lett.}~}
%\def\ps{{Phys. Scr.}~}
%\def\ptch{{Phys. Teach.}~}
\def\ptod{{Phys. Today}~}
%\def\pha{{Physica A}~}
%\def\phb{{Physica B}~}
%\def\phd{{Physica D}~}
%\def\paz{{Pis'ma Astron. Zh.}~}
%\def\pss{{Planet. Space Sci.}~}
%\def\ppcf{{Plasma Phys. Controlled Fusion}~}
%\def\pa{{Postepy Astron.}~}
%\def\pram{{Pram\~{a}na}~}
%\def\pri{{Priroda}~}
%\def\pasa{{Proc. Astron. Soc. Aust.}~}
%\def\pi3e{{Proc. IEEE}~}
%\def\prsl{{Proc. R. Soc. London, Ser. A}~}
%\def\posp{{Proceedings of SPIE}~}
%\def\past{{Prog. Astron.}~}
%\def\ptp{{Prog. Theor. Phys.}~}
%\def\paicas{{Publ. Astron. Inst. Czech. Acad. Sci.}~}
\def\pasj{{PASJ}~} % "Publ. Astron. Soc. Jpn."
\def\pasp{{PASP}~} % "Publ. Astron. Soc. Pac."
%\def\pbao{{Publ. Beijing Astron. Obs.}~}
%\def\pdaub{{Publ. Dep. Astron., Univ. Beogr.}~}
%\def\pdao{{Publ. Dom. Astrophys. Obs.}~}
%\def\pnlaoj{{Publ. Natl. Astron. Obs. Jpn.}~}
%\def\ppmo{{Publ. Purple Mt. Obs.}~}
%\def\psao{{Publ. Shaanxi Astron. Obs.}~}
%\def\pscds{{Publ. Sp\'ec. Cent. Donn\'ees Stellaires}~}
%\def\pyo{{Publ. Yunnan Obs.}~}
%\def\pag{{Pure Appl. Geophys.}~}
%\def\qbsa{{Q. Bull. Sol. Act.}~}
%\def\qjras{{QJRAS}~} % "Q. J. R. Astron. Soc."
%\def\rad{{Radiant}~}
%\def\rsci{{Radio Sci.}~}
%\def\reche{{Recherche}~}
%\def\rpp{{Rep. Prog. Phys.}~}
%\def\ra{{Rev. Astron.}~}
%\def\rg{{Rev. Geophys.}~}
%\def\rmf{{Rev. Mex. Fis.}~}
%\def\rmp{{Rev. Mod. Phys.}~}
\def\rmxaa{{Revista Mexicana de Astronomia y Astrofisica}~}
%\def\rrp{{Rev. Roum. Phys.}~}
%\def\rsi{{Rev. Sci. Instrum.}~}
%\def\rnc{{Riv. Nuovo Cimento}~}
%\def\rh{{\v{R}\'{\i}\v{s}e hv\v{e}zd}~}
%\def\saaoar{{S. Afr. Astron. Obs., Annu. Rep.}~}
%\def\saaoc{{S. Afr. Astron. Obs., Circ.}~}
%\def\saaon{{SAAO Newsl.}~}
%\def\sciam{{Sci. Am.}~}
%\def\scch{{Sci. China, Ser. A}~}
%\def\srtu{{Sci. Rep. T\^{o}hoku Univ., Eighth Ser.}~}
%\def\sc{{Sci}~} % "Science"
%\def\sar{{Sendai Astron. Rap.}~}
%\def\st{{Sidereal Times}~}
%\def\sky{{Sky Telesc.}~}
%\def\sbaavso{{Sol. Bull. (AAVSO)}~}
%\def\se{{Sol. Energy}~}
%\def\sp{{Sol. Phys.}~}
%\def\srd{{Sol. Radio Data}~}
%\def\ssres{{Sol. Syst. Res.}~}
%\def\sdb{{Soln. Dannye, Byull.}~}
%\def\sonne{{Sonne}~}
%\def\sbo{{Soobshch. Byurak. Obs.}~}
%\def\ssao{{Soobshch. Spets. Astrofiz. Obs.}~}
%\def\sost{{South. Stars}~}
%\def\sa{{SvA}~} % "Sov. Astron."
%\def\sal{{SvA}~} % "Sov. Astron. Lett."
%\def\sjot{{Sov. J. Opt. Technol.}~}
%\def\spd{{Sov. Phys. -- Dokl.}~}
%\def\spj{{Sov. Phys. -- JETP}~}
%\def\spu{{Sov. Phys. -- Usp.}~}
%\def\space{{Space}~}
\def\ssr{{Space Sci. Rev.}~}
%\def\stsi{{Space Telesc. Sci. Inst., Newsl.}~}
%\def\sf{{Spaceflight}~}
%\def\sterne{{Sterne}~}
%\def\sw{{Sterne Weltraum}~}
%\def\sb{{Sternenbote}~}
%\def\strlast{{Strolling Astron.}~}
%\def\sgg{{Stud. Geophys. Geod.}~}
%\def\taot{{Tartu Astrof{\"u}{\"u}s. Obs. Teated}~}
%\def\tect{{Tectonophysics}~}
%\def\tellus{{Tellus, Ser. A}~}
%\def\tmf{{Teor. Mat. Fiz.}~}
%\def\tp{{Theor. Pap.}~}
%\def\tsb{{Time Serv. Bull.}~}
%\def\tmnr{{Tokyo Meteor Network Rep.}~}
%\def\tai{{Tsirk. Astron. Inst. (Tashkent)}~}
%\def\ufz{{Ukr. Fiz. Zh.}~}
%\def\ucla{{Universe Classroom}~}
%\def\uao{{Upps. Astron. Obs., Rep.}~}
%\def\urania{{Urania}~}
%\def\usnoc{{U.S. Nav. Obs., Circ.}~}
%\def\usnos4{{U.S. Nav. Obs., Ser. 4}~}
%\def\ufn{{Usp. Fiz. Nauk}~}
%\def\vsb{{Variable Star Bull.}~}
%\def\vasiona{{Vasiona}~}
%\def\varih{{Ver{\"o}ff. Astron. Rechen--Inst. Heidelb.}~}
%\def\vzpe{{Ver{\"o}ff. Zentralinst. Phys. Erde}~}
%\def\vesmir{{Vesm\'{\i}r}~}
%\def\vansssr{{Vestn. Akad. Nauk SSSR}~}
%\def\vku{{Vestn. Kiev. Univ., Astron.}~}
%\def\va{{Vistas Astron.}~}
%\def\wgn{{WGN}~}
%\def\wztud{{Wiss. Z. Tech. Univ. Dresden}~}
%\def\yama{{Yamamoto Circ.}~}
%\def\zap{{Z. Astrophys.}~}
%\def\zamp{{Z. Angew. Math. Phys.}~}
%\def\zna{{Z. Naturforsch., A}~}
%\def\zpa{{Z. Phys., A}~}
%\def\zpc{{Z. Phys., C}~}
%\def\zv{{Zemlya Vselennaya}~}
%\def\zenit{{Zenit}~}
%\def\zetf{{Zh. Ehksp. Teor. Fiz.}~}
\def\procspie{{Proc.~SPIE}~}
